Approximate Query Processing using Deep Generative Models

Data is generated at an unprecedented rate surpassing our ability to analyze them. The database community has pioneered many novel techniques for Approximate Query Processing (AQP) that could give approximate results in a fraction of time needed for computing exact results. In this work, we explore the usage of deep learning (DL) for answering aggregate queries specifically for interactive applications such as data exploration and visualization. We use deep generative models, an unsupervised learning based approach, to learn the data distribution faithfully such that aggregate queries could be answered approximately by generating samples from the learned model. The model is often compact - few hundred KBs - so that arbitrary AQP queries could be answered on the client side without contacting the database server. Our other contributions include identifying model bias and minimizing it through a rejection sampling based approach and an algorithm to build model ensembles for AQP for improved accuracy. Our extensive experiments show that our proposed approach can provide answers with high accuracy and low latency.

==> extensions.tex <==
\section{Extensions}
\label{sec:extensions}

So far, we had focused on VAE as the generative model as it is especially well suited for AQP.
In this section, we consider two other generative models : 
Generative Adversarial Networks (Section~\ref{subsec:GANforAQP})
and Bayesian Networks (Section~\ref{subsec:DBNforAQP}).
The three models have their own comparative advantages and disadvantages that we describe in Section~\ref{subsec:comparativeAnalysisForAQP}.
In Section~\ref{subsec:conditionalGeneration}, we describe how to directly generate samples that satisfy a given query. 

\subsection{AQP using Generative Adversarial Networks}
\label{subsec:GANforAQP}

\stitle{GAN Primer.}
Generative Adversarial Networks (GANs)~\cite{} are a popular and powerful class of generative models that seek to 
\emph{implicitly} minimize the divergence between true and generative model's probability distribution.
They consist of two major components.
The \emph{generator} takes in noise vectors and outputs sample tuples that could have been produced by the true probability distribution.
The \emph{discriminator} seeks to classify whether a given tuple is true (\ie from the true probability distribution) 
or fake (\ie produced by generator's probability distribution).
Hence, this could be considered as a game where the generator tries to generate realistic tuples that could fool the discriminator.
In turn, the discriminator tries to maximize the chance or correctly determining if the tuple is true or fake.
Over an ideal training process, both the generator and discriminator become increasingly better 
with the generator producing tuples that are indistinguishable from the tuples from the underlying dataset. 
For additional details, please refer to the tutorial~\cite{}.

%Intuitively, in order to generate good fake tuples, the generator must understand how the real data looks like.
%To make this challenging, only the discriminator has access to the underlying dataset. 
%Hence, the generator must learn to generate samples that could have come from the true distribution without having access to it.
%It does this by \emph{implicitly} learning the probability distribution.
%It begins by generating a random noise vector and learning an appropriate transformation such that it gets converted to a tuple.
%We can see that the random vector acts as a latent code (similar to the output of VAE's encoder).

\stitle{GAN for AQP.}
We begin by encoding the input tuples using the same techniques as for VAE. 
The generator generates random noise vectors according to a noise probability distribution and learns to transform them into sample tuples.
The discriminator is fed with a random sample of tuples from the real dataset as positive examples and
the tuples from the generator as negative examples.
The discriminator then uses these positive and negative examples to discern which of the examples were generated by the generator.
Initially, the task of discriminator is easy as generator outputs nonsensical tuples.
However, as the generator inputs, the task becomes more and more challenging.
Note that the discriminator is trained on the latest samples from the generator - so the discriminator also improves.
If an equilibrium is achieved, the samples produced by generator are virtually indistinguishable from the true dataset.
Once such a model is trained, it could be used for generating samples and answer AQP queries.
Specifically, we generate random noise vectors based on the noise distribution and use the generator to transform them into tuples. 
The synthetic tuples that are generated could be transparently used for AQP purposes. 

Even though they are conceptually appealing, GANs are notoriously hard to train and suffer from 
various issues such as mode collapse and non convergence~\cite{tutorial}. 
In our paper, we used Wasserstein GAN~\cite{} as it has improved convergence properties. 
Please refer to Section~\ref{subsec:comparativeAnalysisForAQP} for additional discussion comparing GANs with VAEs.

\subsection{AQP using Bayesian Networks} 
\label{subsec:DBNforAQP}

\stitle{Bayesian Network Primer.}
(Deep) Bayesian networks (BN) are another effective generative model that elegantly combines probability and graph theory.
A Bayesian network is a directed acyclic graphical structure where nodes correspond to random variable $A_i$ (for attribute $A_i$)
and directed edges between nodes signify (direct) dependencies between the corresponding attributes.
For the sake of exposition, we assume that all attributes are discrete. 
However, BNs are capable of handling a mixture of discrete and continuous variables. 
Given an edge $A_i \rightarrow A_j$, $A_i$ is the parent of $A_j$.
Any node without parents is called as a root node while other nodes are called intermediate nodes.
Each node is associated with a conditional probability table (CPT) involving itself and its parents.
Let $A_i$ and $A_j$ be two Boolean variables with $A_i$ being the parent of $A_j$.
If $A_i$ is a root node, then the CPT of $A_i$ has two entries for $P(A_i=0)$ and $P(A_i=1)$ involving itself. 
The CPT of $A_j$ has four entries corresponding $P(A_j=0|A_i=0), \ldots, P(A_j=1|A_i=1)$.
Given this setting, BNs represent the joint distribution of any combination of variables as 
\begin{equation}
	P(A_1, A_2, \ldots, A_n) = \prod_{i=1}^{n} P(A_i| Parents(A_i))
	\label{eq:bnJPD}
\end{equation}

\stitle{BN for AQP.}
Using BN for AQP is fairly straightforward.
We begin by creating a graph with $n$ nodes and no edges.
Note that unlike VAE or GANs, we do not need to perform any input encoding for BN.
The goal of \emph{structure learning}~\cite{} is to learn the topology of BN (i.e. the connectivity between nodes) and
the CPT for each node that best explains the dataset $T$.
Learning the optimal BN topology is a NP-complete problem~\cite{}
However, there exists a number of efficient heuristic algorithms that 
start with an empty BN and iteratively adds edges that maximizes a scoring function. 
Please refer to~\cite{} for a detailed discussion.
The learned BN approximates the underlying data distribution using Equation~\ref{eq:bnJPD} and could be used to generate samples.
Traditional AQP techniques could be applied on the samples to generate estimates. 

\stitle{Sampling from Bayesian Networks.}
For each root node, we generate its value based on its prior probability distribution specified in its CPT. 
Then for each intermediate node, we condition them based on the attribute values chosen for their parents,
choose the corresponding entry in CPT and randomly sample its value from probability distribution.
Consider a simple BN from Figure~\ref{fig:sampleBN} from which we can generate a sample $t$ as follows.
First, we consider the root nodes $A_1$ and $A_2$.
We select the value of $t[A_1]$ using the CPT of $A_1$.
Specifically, we set $t[A_1]$ to 0 with probability $0.6$ and $1$ with probability $0.4$.
Similarly, we set $t[A_2]$ to $0$ with probability $0.1$ and $1$ otherwise.
Let the selected values be $t[A_1]=1, t[A_2]=0$.
From the CPT of $A_3$, we can see that when when $t[A_1]=1, t[A_2]=0$, $t[A_3]=0$ with probability $0.4$ and $1$ with probability $0.6$.
We generate the value for $t[A_3]$ (say $1$) based on this distribution.
Then the tuple $t = [1, 0, 1]$ is the sample generated from the BN.
One could repeat the process to generate as many samples as necessary and apply the traditional AQP techniques over the samples. 

\begin{figure}[h!]
	\centering
	\includegraphics[scale=0.35]{figures/Blank.png}
	\caption{Sampling from a Bayesian Network}
	\label{fig:sampleBN}
\end{figure}

\stitle{Likelihood Weighting for Conditional Samples.}
It is also possible to generate conditional samples where some attributes are set to a specific value.
Let $\{A_i, A_j, \ldots\}$ be the set of variables for which we fixed the values $\{a_i, a_j, \ldots\}$ respectively. 
In other words, we are only interested in samples $A_i=a_i$ and so on.
This could be achieved by \emph{likelihood weighting} where we fix the value of sample's $A_i, A_j, \ldots$ to $a_i, a_j, \ldots$ and 
use the aforementioned process for generating samples for other variables.
However, note that this is not a uniform random sample.
Instead, its likelihood is computed by weighting by probability of $A_i, A_j, \ldots$ given the value of its parents.

\red{TBD. Give a worked out example based on the example.}


\subsection{Conditional Generation of Samples}
\label{subsec:conditionalGeneration}

So far, we have focused on \emph{unconditional} generative models that learn the underlying data distribution
and generate uniform random samples from the variational posterior.
We next describe an efficient approach to generate \emph{biased} samples that satisfy the given query.
Traditional AQP techniques for generating unbiased estimates from biased samples could be used without any modifications.

\stitle{Need for Conditional Generation.}
While uniform random samples could be used to estimate aggregates for any query,
there are many scenarios where this approach is inefficient.
Common examples include queries with low selectivity or aggregates over GROUP-BY operators. 
Consider a query $q$ whose selectivity is $0.1\%$. 
On expectation, only $1$ out of every $1000$ uniformly generated samples satisfy $q$. 
Hence, we need to generate thousands of samples before we have sufficient number of samples that satisfy $q$ that could be used to provide accurate estimates.
All the samples that does not satisfy $q$ are simply discarded. 
A better strategy is to only generate samples that satisfy $q$ thereby minimizing waste by not discarding irrelevant samples. 
This approach also makes aggregates over GROUP-BY queries more efficient.
Specifically, we only generate relevant samples for each of the groups returned by the query. 
In traditional AQP, the biased samples are often pre-computed by analyzing the workload~\cite{garofalakis2001approximate,mozafari2015handbook}.
If the queries deviate from the workload, they could incur larger approximation errors. 
In contrast, we could generate conditional samples during the runtime in response the input query. 

\stitle{Conditional Generation for VAE and GANs.}
We had previously described the likelihood weighting approach for conditional generation for BNs.
We now describe a efficient mechanism to generate conditional samples for VAE for GANs.
This approach could be used for AQP if we know that most of the queries involving filtering over the same set of 2-3 attributes. 
For example, most of the queries to an enterprise data warehouse could involve year or country. 
In this scenario, it is possible to design conditional variants for generative models such as VAE~\cite{} and GANs~\cite{}. 

We now briefly describe a popular and canonical approach - Conditional Variation Auto Encoder (CVAE)~\cite{cvaepaper,attrConditioningImageGenPaper}.
The intuition for conditional GANs is similar.
Recall that VAE involves two components: encoder $q(z|X)$ and decoder $p(X|z)$ - both of which does not take into account any conditions. 
The key idea behind CVAE~\cite{cvaepaper} is to introduce random variable(s) $Y$ (typically called labels or conditions) 
that could be used to condition the data generation process. 
In other words, the encoder is now conditioned on $q(z|X,y)$ where $y \in Y$ and decoder is conditioned on $q(z|X,y)$.
Finally, the prior distribution of the latent variables $p(z)$ is also now conditioned on $y$; \ie $p(z|y)$ for each $y \in Y$. 
The rest of the derivation is identical to that VAE.
For example, one could train a CVAE~\cite{attrConditioningImageGenPaper} by training it on images 
for which additional labels/conditions such as the age, gender, facial expression etc are also provided.
Then given a condition such as \emph{y = \{age=young, gender=male, expression=smiling\}}, 
one could generate a sample from the distribution $p(z|y)$ and then pass it to parameterized decoder $p(X|y,z)$. 

%\stitle{Approach 2: Conditional Generation using Latent Subspaces.}
%Conditional generative models are an effective strategy when the conditions involved are limited.
%However, if the conditions are complex (\eg involving many attributes) or numerous (\eg it might involve many combinations of attributes),
%this requires expensive retraining to create new conditional models.
%Suppose the AQP system could get queries with predicates specified over: (a) only year (b) only country or (c) both year and country.
%We have to train one conditional model for each of these scenarios thereby requiring three CVAE models overall. 

\subsection{Comparative Analysis of Generative Models for AQP.}
\label{subsec:comparativeAnalysisForAQP}

\begin{itemize}
	\item Make sure justification are in abstract, intro and other places.
	\item Justify why these three models were chosen
	\item Justify why focus was on VAE
	\item pros and cons of these
\end{itemize}




